Simple Dynamic Spanners with Near-optimal Recourse against an Adaptive Adversary

Designing dynamic algorithms against an adaptive adversary whose performance match the ones assuming an oblivious adversary is a major research program in the field of dynamic graph algorithms. One of the prominent examples whose oblivious-vs-adaptive gap remains maximally large is the \emph{fully dynamic spanner} problem; there exist algorithms assuming an oblivious adversary with near-optimal size-stretch trade-off using only $\operatorname{polylog}(n)$ update time [Baswana, Khurana, and Sarkar TALG'12; Forster and Goranci STOC'19; Bernstein, Forster, and Henzinger SODA'20], while against an adaptive adversary, even when we allow infinite time and only count recourse (i.e. the number of edge changes per update in the maintained spanner), all previous algorithms with stretch at most $\log^{5}(n)$ require at least $\Omega(n)$ amortized recourse [Ausiello, Franciosa, and Italiano ESA'05]. In this paper, we completely close this gap with respect to recourse by showing algorithms against an adaptive adversary with near-optimal size-stretch trade-off and recourse. More precisely, for any $k\ge1$, our algorithm maintains a $(2k-1)$-spanner of size $O(n^{1+1/k}\log n)$ with $O(\log n)$ amortized recourse, which is optimal in all parameters up to a $O(\log n)$ factor. As a step toward algorithms with small update time (not just recourse), we show another algorithm that maintains a $3$-spanner of size $\tilde O(n^{1.5})$ with $\operatorname{polylog}(n)$ amortized recourse \emph{and} simultaneously $\tilde O(\sqrt{n})$ worst-case update time.

==> header_arxiv.tex <==

\usepackage{amsmath,amsthm,amsfonts}
% \usepackage{fullpage}
\usepackage{comment}
\usepackage{array}
\usepackage{verbatim}
\usepackage{float}
\usepackage{multirow}
\usepackage{enumitem}
\usepackage{fontspec}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{thm}[theorem]{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{invariant}[theorem]{Invariant}


\usepackage{xcolor}
\usepackage{nameref}
Nicer hyperref obtained from Babis
\definecolor{ForestGreen}{rgb}{0.1333,0.5451,0.1333}
\definecolor{DarkRed}{rgb}{0.8,0,0}
\definecolor{Red}{rgb}{1,0,0}
\usepackage[linktocpage=true,
pagebackref=true,colorlinks,
linkcolor=DarkRed,citecolor=ForestGreen,
bookmarks,bookmarksopen,bookmarksnumbered]
{hyperref}
\usepackage{cleveref}
\usepackage{mathtools}
\usepackage{thmtools}

% \usepackage[showframe=true]{geometry} % Just for fixing position. comment out on submission.
\usepackage{changepage}


\declaretheorem[numberwithin=section]{theorem}
\declaretheorem[numberlike=theorem]{lemma}
\declaretheorem[numberlike=theorem,name=Lemma]{lem}
\declaretheorem[numberlike=theorem]{proposition}
\declaretheorem[numberlike=theorem,name=Proposition]{prop}
\declaretheorem[numberlike=theorem]{corollary}
\declaretheorem[numberlike=theorem,name=Corollary]{cor}
\declaretheorem[numberlike=theorem,style=definition]{definition}
\declaretheorem[numberlike=theorem,style=definition,name=Definition]{defn}
\declaretheorem[numberlike=theorem]{claim}
\declaretheorem[numberlike=theorem]{fact}
\declaretheorem[numberlike=theorem]{observation}
\declaretheorem[numberlike=theorem,name=Observation]{obs}
\declaretheorem[numberlike=theorem]{invariant}
\declaretheorem[numberlike=theorem,name=Invariant]{inv}
\declaretheorem[numberlike=theorem,style=remark]{remark}
\declaretheorem[numberlike=theorem,style=remark,name=Remark]{rem}
\declaretheorem[numberlike=theorem,style=definition]{goal}
\declaretheorem[numberlike=theorem]{assumption}
\theoremstyle{remark}
\newtheorem*{rem*}{Remark}


\newcommand{\eps}{\epsilon}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\eqdef}{\overset{{\mathrm {\footnotesize def}}}{=}}
\newcommand{\cpy}{c}
\newcommand{\vol}{vol}
\newcommand{\density}{\rho}
\newcommand{\profit}{v}

%LP environment stuff
\newcommand{\mini}[1]{\mbox{minimize} & {#1} &\\}
\newcommand{\maxi}[1]{\mbox{maximize} & {#1 } & \\}
% \newcommand{\st}{\mbox{subject to} }
\renewcommand{\st}{\mbox{subject to} }
\newcommand{\con}[1]{&#1 & \\}
\newcommand{\qcon}[2]{&#1, & \mbox{for } #2.  \\}
\newenvironment{lp}{\begin{equation}  \begin{array}{lll}}{\end{array}\end{equation}}
\newenvironment{lp*}{\begin{equation*}  \begin{array}{lll}}{\end{array}\end{equation*}}

\providecommand{\tabularnewline}{\\}
% \floatstyle{ruled}

\global\long\def\Otil{\tilde{O}}
\global\long\def\polylog{\operatorname{polylog}}
\global\long\def\poly{\operatorname{poly}}
\global\long\def\dist{\operatorname{dist}}



\newcommand{\F}{\mathcal{F}}
\renewcommand{\S}{\mathcal{S}}
\providecommand{\U}{\mathcal{U}}
\renewcommand{\U}{\mathcal{U}}
\newcommand{\B}{\mathcal{B}}
\providecommand{\C}{\mathcal{C}}
\renewcommand{\C}{\mathcal{C}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\d}{\mathrm{deg}}
\renewcommand{\P}{\mathbb{P}}

\newcommand{\job}{\mathrm{job}}
\newcommand{\target}{\mathrm{target}}
\newcommand{\Sampling}{\textsc{Resample}}
\newcommand{\Resample}{\textsc{Resample}}
\newcommand{\ind}{\mathrm{ind}}
\newcommand{\Schedule}{\textsc{Schedule}}
\renewcommand{\exp}{\mathrm{exp}}

\newcommand{\prt}{\mathrm{prt}}
\newcommand{\parent}{\mathrm{parent}}
\newcommand{\children}{\mathrm{children}}
\newcommand{\ppath}{\mathrm{path}}
\newcommand{\dest}{\mathrm{dest}}
\newcommand{\level}{\mathrm{level}}
\newcommand{\new}{\mathrm{new}}
\newcommand{\old}{\mathrm{old}}



% Author comments
\def\ShowComment{True} % Switch comments  on or  off

\ifdefined\ShowComment
\def\thatchapholtext#1{\textcolor{purple}{#1}}
\def\thatchaphol#1{\marginpar{$\leftarrow$\fbox{T}}\footnote{$\Rightarrow$~{\sf\textcolor{purple}{#1 --Thatchaphol}}}}
\def\pattext#1{\textcolor{purple}{#1}}
\def\pat#1{\marginpar{$\leftarrow$\fbox{P}}\footnote{$\Rightarrow$~{\sf\textcolor{red}{#1 --Pat}}}}


\else
\def\thatchapholtext#1{}
\def\thatchaphol#1{}
\def\pattext#1{}
\def\pat#1{}

\fi


==> three_spanner.tex <==
%!TEX root=writeup.tex
\section{$3$-Spanner with worst-case time}\label{sec:3-spanner}




In this section, we show how to maintain $3$-spanner deterministically with a good running time.

\begin{theorem}\label{lemma:3-spanner_guarantee}
    There exists a deterministic algorithm that maintain a $3$-spanner of size
    $\tilde O(  n \sqrt{n})$
    % in a decremental graph against an adaptive adversary.
    in a fully-dynamic graph.
    The preprocessing time of the algorithm is $O((m+n) \log n)$
    and the worst-case update time is $O(\sqrt{n} \log{n} )$ per edge update.

\end{theorem}

To show the theorem above, we begin by describing our spanner construction in static manner.
Let $G = (V,E)$ be the given graph, we construct $H = (V, F \subseteq E_H)$ such that
$\dist_H(u,v) \leq 3~\dist_G(u,v)$.

\paragraph*{Notations:} For any graph $G = (V,E)$, we let $E(S,T) = \{e= (u,v) \in E : u \in S, v \in T\}$
be the set of edges connecting vertices in $S$ to vertices in $T$. When $S =\{u\}$ ($T = \{v\}$),
is a single vertex, we may drop the bracket and use $E(u,T)$ ($E(S,v)$) instead.
In our construction, we will partition $V$ into $\sqrt{n}$ \emph{buckets},
each of size $\Theta(\sqrt{n})$. We call these buckets $V_1, V_2, \ldots, V_{\sqrt{n}}$.
Note that since this is a partition of $V$, $V_i \cap V_{j\neq i} = \emptyset$ and $\bigcup_i V_i = V$.
For all vertex $v$, let $b(v)$ be the bucket that $v$ belongs to.


%
% For any node $u \notin V_i$, we let $c_i(u)$ be the node $v$ such that $v \in V_i$ and $u \in C_v$.
% If $u \in V_i$, we let $c_i(u) = u$. We let $C^+_v = C_v \cup \{v\}$ be the cluster of vertices centered at $v$, including $v$.



\paragraph*{Static construction:}
As mentioned above, we first partition $V$ into $\sqrt{n}$ \emph{buckets} $V_1 \ldots, V_{\sqrt n}$.
% each of size $\Theta(\sqrt{n})$. We call these buckets $V_1, V_2, \ldots, V_{\sqrt{n}}$.
% Note that since this is a partition of $V$, $V_i \cap V_{j\neq i} = \emptyset$ and $\bigcup_i V_i = V$.
For every buckets, we do the following.
On bucket $i$, for each $v \notin V_i$, if $E(v, V_i)$ is not empty,then we pick $e = (v,c_i(v)) \in E(v,V_i)$
and insert $e$ to $E_H$. We call these edges \emph{type-$1$} edges.
For $u \in V_i$, let $\C (u)$ be the set of vertices in $V \setminus V_i$ connecting to $u$ via type-$1$ edges.
For convenience, we also let $\C^+(u) = \C (u) \cup \{u\}$.
$\C(u)$ ($\C^+(u)$) is a \emph{cluster} of vertices centered at $u$.
For all $v$, we let $c_i(v)$ be the center of the cluster $v$ belongs to in $V_i$.
If $E(v, V_i)$ is empty, then $c_i(v) = \null$ and if $v \in V_i$, then $c_i(v) = v$.
Now we describe \emph{type-$2$} edges.
For all $u,u' \in V_i$, if $E(u, \C^+(u'))$ is not empty,
then we pick one edge $e_{u,u'}$ from this set and insert it to $E_H$.
$e_{u,u'}$ is a type-$2$ edge connecting $u$ to $\C^+(u')$, the cluster centered at $u'$. This is the whole construction.


\begin{claim}
    Let $H = (V,E_H)$ be the graph produced by our construction above, then $H$ is a $3$-spanner of size $O(n \sqrt{n})$.
\end{claim}
\begin{proof}
    We first show that $|E_H| = O(n \sqrt{n})$. Consider bucket $i$.
    Since any vertex in $V \setminus V_i$ contribute at most one type-$1$ edge to bucket $i$, there are $O(n)$ type-$1$ edges in bucket $i$.
    Since $|V_i| = \Theta(\sqrt n)$, and we have at most one type-$2$ edge for each pair $u,u' \in V_i$,
    there are at most $O(n)$ type-$2$ edges for bucket $i$. Since we have exactly $\sqrt n$ buckets, $|E_H| = O(n \sqrt {n})$.

    We now argue that $H$ is a $3$-spanner. For any edge $e =(u,v) \in E_H$,
    it is obvious that $\dist_H(u,v) \leq 3$. Suppose $e = (u,v) \notin E_H$,
    let $i = b(v)$. Because $(u,v) \in E$, $E(u,V_i)$ is not empty.
    Hence, there exists $u' \in V_i$ such that $(u,u')$ is a type-$1$ edge in $E_H$.
    Since $u \in \C (u')$, $E(v, \C^+(u'))$ is not empty, hence,
    there exists $v' \in \C^+(u')$ such that $(v, v')$ is a type-$2$ edge in $E_H$.
    Note that since $(u,v) \notin E_H$, it cannot be the case that $u' = v$ os $v' = u$.
    Consider the path $u-u'-v'-v$, this is a $u-v$ path of length at most $3$
    (if $u'=v'$, the this path has length 2), hence $\dist_H(u,v) \leq 3$. This conclude the proof.
\end{proof}

% \paragraph*{CONGEST: }Our static construction can be implemented in CONGEST model in two rounds.

It is not hard to see that our static construction can be implemented in CONGEST model.

\begin{corollary}
    The construction can be implemented in CONGEST model in two rounds.
\end{corollary}
\begin{proof}
In the first round, for every vertex and every bucket, the vertex pick a cluster that they belong to. In the second round, for every vertex and every bucket, the vertex broadcasts
the cluster it belongs to to other adjacent vertices in that bucket. Each vertex then picks type-$2$ edges to complete the construction.

\end{proof}

% \subsection{Maintain Spanner in the decremental setting}
\subsection{Maintain Spanner in the fully-dynamic setting}

\paragraph*{Data structure:} For all $v$ and for all $i$, we need to maintain $E(v, V_i)$.
We also need to maintain $E(u, \C^+(u'))$ for all $u,u' \in V_i$.
These sets of edges will be maintained using a balanced binary search tree.
Hence, we assume that we can insert, delete, and find a vertex (or an edge)
in $O(\log n)$ time.
For each edge, we need to know which type(s) it is and how it is used for, e.g.,
$e$ is a type-$1$ edge connecting $v$ to $V_i$ and/or $e$ is a type-$2$ edge
connecting $u$ to $\C^+(u')$. This information will be needed when $e$ is deleted,
as it will tell us what edges we need to find. The work of adding these information
to an edge can be charged to the time we add $e$ to $E_H$.

\paragraph*{Preprocessing:} We follow closely what we described in \textbf{Static construction}.
We first partition $V$ into $\sqrt n$ buckets.
This can be done in $O(n)$ time.
We then maintain $E(v, V_i)$ for all $v, i$ and select one type-$1$ edge for all $v,i$
At this point $\C (v)$ and $\C^+(v)$ are defined for all $v$.
We maintain $E(u, \C^+(u'))$ for all $u,u' \in V_i$ and select one type-$2$ edge for all
$u,u' \in V_i$, for all $i$. It is easy to see that
all the steps can be done in $O((m+n) \log n)$.


To deterministically maintain our spanner, it
suffices to show how we can maintain type-$1$ and type-$2$ edges. We devote the rest of the section to show
that we can maintain these edges with $O(\sqrt{n} \log n)$ update time.

\paragraph*{Handle edge deletions:} Let us inspect what could happen when an edge gets deleted.
The easiest case is when the edge $e = (u,v)$ that is deleted is a non-spanner edge, i.e., $e \notin E_H$.
In this case, we don't have to add anything to $E_H$.

% Make the two paragraph*s below precise.
\paragraph*{Handle type-$1$ edge deletion:}
Suppose $e = (u,v)$ is a type-$1$ edge, WLOG, assume that $u \in \C(v)$ and $i = b(v)$.
Since $e$ is an edge connecting $u$ to $V_i$, we have to find a replacement edge in $E(u, V_i)$.
If there is such an edge $e' = (u, v')$ where $b(v') = i$, then we add $e'$ to $E_H$.
Removing a type-$1$ edge can affect the usability of type-$2$ edges.
For example, suppose there exists $w \in V_i$, such that $e_w = (w,u)$ is a type-$2$ edge
connecting $w$ to $\C^+(v)$ in $E_H$. In this case, we need to find a replacement
edge in $E(w, \C^+(v))$, if any. We also need to remove $e_w = (w,u)$ from $E_H$ if
there is already an edge $e^\prime_w \in E(w,\C^+(v'))$ connecting $w$ to $\C^+(v')$.
As there could be $O(|V_i|) = O(\sqrt{n})$ such $w$, this might cause
up to $O(\sqrt{n})$ insertions and deletions.

\paragraph*{Handle type-$2$ edge deletion:}
Suppose $e = (u,v)$ is a type-$2$ edge in phase $i = b(v)$.
Let $w = c_i(u)$, then $e$ is a type-$2$ edge connecting $v$ to $\C^+(w)$.
In this case, we need to find an alternate edge connecting $v$ to $\C^+(w)$.
To fix this connection, we pick one of the remaining edges in $E(v,\C^+(w))$
and add it to $E_H$. If there is no such edge, then we do nothing.

% It is easy to observe that using the datastructure .... this can be implemented in O(..)

Let us remark that an edge $e = (u,v)$ can be both type-$1$ and type-$2$ at the same time.
It can also be, for example, type-$1$ edge connecting $u$ to $v \in V_i$ and connecting $v$ to $u \in V_j$.
However, this is fine as the amount of work we need to fix is blown up by at most constant times in a phase
and $e$ can only appear in at most two phases (the one where $u$ is a member of, and the one where $v$ is a
member of).
% Do we need a formal claim for this?

\paragraph*{Handle edge insertions:} For an edge inserted by an adversary, we need to check if the inserted edge $e= (u,v)$
should be used as type-$1$ edge or type-$2$ edge (or both). Let $i = b(u),j = b(v)$.
If $e$, which is just inserted, is the only edge in $E(u,V_j)$ (resp, $E(v, V_i)$),
then we have to add $e$ to $E_H$ and $e$ would be a type-$1$ edge.
Let $v' = c_i(v)$ and $u' = c_j(u)$, if $e$ is the only edge in
$E(u, \C^+(v'))$ (resp, $E(v, \C^+(u'))$), then we add $e$ to $E_H$ as a type-$2$ edge.

\begin{observation}\label{obs:insertion_bound}
    An edge deletion by an adversary can cause at most $O(\sqrt{n})$ edge insertions and edge deletions.
\end{observation}

% \subsection{Implementation}\label{subsect:implementation}
%
% To prove Lemma~\ref{lemma:3-spanner_guarantee}, we need to be able to locate what we need to fix and update edges in
% time $O(\log n)$ per edge. This subsection is devoted to show exactly how to implement the $3$-spanner.
% Every step can be done using standard data structures.
% In particular, we want to maintain a list where we can insert, delete, or find a specific object in $O(\log n)$,
% this can be implemented with a standard balanced binary search tree. For simplicity, when we say a \emph{list},
% we refer to this structure that support efficient insertion, deletion, and element finding.
%
% \paragraph*{Initialization:} We first need to partition $V$ into $V_1, \ldots, V_{\sqrt n}$. Since this
% can be done arbitralily, we can partition vertices in $O(n)$ times.
% For each vertex $v$, we want to group edges adjacent to $v$ so that
% we know which edges lead $v$ to which phases.
% More formally, we want to maintain $E(v, V_i)$ for all $i$.
% This can be done in total time $O((n+m) \log n)$.
% More formally, for all phase $V_i$, and for all vertex $v \in V \setminus V_i$,
% we maintain a list for $E(v,V_i)$.
% Then, we establish type-$1$ edges, that is, for all phase $V_i$ and for all vertex $v \in V \setminus V_i$,
% we pick an edge $e$ from $E(v,V_i)$ and add $e$ to $E_H$. This can be done in $O( (n+m) \log n)$.
% Finally, we establish type-$2$ edges. For each $u,v \in V_i$, we want to maintain the list $E(u, C^+_v)$.
% To do this, we can go over each vertex $w \in V \setminus V_i$, and for each $(w,x) \in E(w,V_i)$, we
% add to $E(x, C^+_v)$, the edge $(w,x)$. These initialization is again can be done in $O( (n+m) \log n)$
% as we only need to traverse the list of edges once. We then select one edge $e \in E(u, C^+_v)$ for each
% pair of vertices $u,v \in V_i$, and for all $v_i$. This part can be done in $(n \sqrt{n} \log n)$.
% This concludes our initialization.
%
% \paragraph*{Handle edge insertion:} When an edge $e = (u,v)$ is inserted, we do the following.
% Let $i,j$ be such that $u \in V_i$ and $v \in V_j$. We add $e$ into $E(u, V_j)$ and $E(v, V_i)$.
% If $e$ be the only edge in $E(u, V_j)$, (resp, $E(v, V_i)$), then we add $e$ into
% $E_H$, in this case, $e$ will be a type-$1$ edge connecting $u$ to $V_j$, (resp, $v$ to $V_i$).
% Now we let $v' = c_i(v)$ ($u' = c_j(u)$). If $v' \neq u$ (resp, $u' \neq v$),
% we add $e$ into $E(u, C^+_{v'})$, (resp, $E(v, C^+_{u'})$). Adding $e$ into each set can be
% done in $O(\log n)$, hence we spend $O(\log n)$ time for each edge insertion.
%
%
% \paragraph*{Handle non-spanner edge deletion:} Let us consider the easiest case. Suppose
% an edge $e =(u,v)$ deleted by the adversary is not a spanner edge. While it is true that
% we do not have to make any changes to $E_H$, we still have to maintain our data structure.
% Consider $V_i \ni v$, we have to delete $e$ from the list $E(u, V_i)$.
% %Likewise, we have to delete $e$ from the list $E(v, V_j \ni u)$.
% If $u \in C^+_{v'}$ where $v' \in V_i$, then we have to delete $e$ from $E(v, C^+_{v'})$.
% Symmetrically, we have to do the same work in $V_j \ni u$. Each of these deletion can be done
% in $O(\log n)$, hence the update time for non-spanner edge deletin is $O(\log n)$.
%
% We note that the procedure above, which maintain the required information when
% deleting a non-spanner edge, will also be applied to spanner edges.
% % This is a prerequisite, how should I state this?
%
% \paragraph*{Handle type-$1$ edge deletion:} Wlog, for the deleted edge $e= (u, v)$,
% assume that $u \in C^+_v$ and $v \in V_i$. Let $v_1 v_2 \ldots v_{\sqrt{n} - 1}$ be
% vertices in $V_i \setminus \{v\}$. We first check if $E(u, V_i)$ is empty.
% If not, then we select $j$ such that $(u, v_j) \in E(u,V_i)$ and add it to $E_H$.
% This can be done in $O(\log n)$ as $j$ can be chosen arbitrarily.
% As mentioned above, this can affect functionality of up to $O(\sqrt {n})$
% type-$2$ edges. For $1 \leq \ell \leq \sqrt{n} -1$, we do the following,
% (1) we check if $(u, v_\ell)$ is the type-$2$ edge connecting $v_\ell$ to
% $C^+_v$. If that is the case, then we remove $(u, v_\ell)$ from $E_H$
% and find another edge $e' \in E(v_\ell, C^+_v)$ and add it to $E_H$.
% This can be done in $O(\log n)$. (2) We then check if we already have
% a type-$2$ edge between $v_\ell$ and $C^+_{v_j}$. If not, and if
% $(u, v_\ell) \in E$, then we add $(u, v_\ell)$ to $E_H$ so
% this edge becomes the type-$2$ edge connecting $v_\ell$ to $C^+_{v_j}$.
% This part can also be done in $O(\log n)$.
% Since we have to do the checking for $O(\sqrt {n})$ vertices,
% the worst case update time is $O(\sqrt {n} \log n)$ per type-$1$ edge deletion.
%
% \paragraph*{Handle type-$2$ edge deletion:} Wlog, for the deleted edge $e= (u,v)$,
% assume that $u \in C^+_w$ and $w,v \in V_i$, i.e., $e$ is a type-$2$ edge connecting
% $v$ to $C^+_w$ in $V_i$ (it could be that $w=u$). In this case, we remove $e$ from $E(v, C^+_w)$.
% After that, if $E(v, C^+_w)$ is still not empty, then we pick an edge $e' = (u',v) \in E(v,C^+_w)$
% and add it to $E_H$. Note that removing $e$ from $E(v, C^+_w)$ and finding $e'$ takes $O(\log n)$ each.
% Hence, in total, we can handle a type-$2$ edge deletion in $O(\log n)$.
%
% This concludes our algorithm. To recap, Observation~\ref{obs:insertion_bound}
% is used to bound the number of edge insertions and edge deletions per
% an adversary deletion. To achieve the desired running time, as in Lemma~\ref{lemma:3-spanner_guarantee},
% we describe what information we need to maintain and how to maintain them in Subsection~\ref{subsect:implementation}.
% Combining them gives us Lemma~\ref{lemma:3-spanner_guarantee}.

